SaSTL: Spatial Aggregation Signal Temporal Logic for Runtime Monitoring in Smart Cities

We present SaSTL -- a novel Spatial Aggregation Signal Temporal Logic -- for the efficient runtime monitoring of safety and performance requirements in smart cities. We first describe a study of over 1,000 smart city requirements, some of which can not be specified using existing logic such as Signal Temporal Logic (STL) and its variants. To tackle this limitation, we develop two new logical operators in SaSTL to augment STL for expressing spatial aggregation and spatial counting characteristics that are commonly found in real city requirements. We also develop efficient monitoring algorithms that can check a SaSTL requirement in parallel over multiple data streams (e.g., generated by multiple sensors distributed spatially in a city). We evaluate our SaSTL monitor by applying to two case studies with large-scale real city sensing data (e.g., up to 10,000 sensors in one requirement). The results show that SaSTL has a much higher coverage expressiveness than other spatial-temporal logics, and with a significant reduction of computation time for monitoring requirements. We also demonstrate that the SaSTL monitor can help improve the safety and performance of smart cities via simulated experiments.

==> 8_discussion.tex <==
% \section{Discussion}
\label{sect:dis}

While we believe that the work presented here is a major advance to the state of art, there are still open questions. Today, most smart cities do employ a centralized dashboard solution similar to the model we assume. As cities and services grow, a more decentralized model may be necessary. However, the solution presented here can be decentralized by creating a hierarchy of monitors. 

The use of a monitor like SaSTL to predict future violations is strongly dependent on the quality and accuracy of the model of city performance. In the second case study of this work we used SUMO which was developed by the transportation community over many years and is considered state of the art. Developing more comprehensive and accurate models is necessary, but is orthogonal to this work.


